FlowMM: Generating Materials with Riemannian Flow Matching

Crystalline materials are a fundamental component in next-generation technologies, yet modeling their distribution presents unique computational challenges. Of the plausible arrangements of atoms in a periodic lattice only a vanishingly small percentage are thermodynamically stable, which is a key indicator of the materials that can be experimentally realized. Two fundamental tasks in this area are to (a) predict the stable crystal structure of a known composition of elements and (b) propose novel compositions along with their stable structures. We present FlowMM, a pair of generative models that achieve state-of-the-art performance on both tasks while being more efficient and more flexible than competing methods. We generalize Riemannian Flow Matching to suit the symmetries inherent to crystals: translation, rotation, permutation, and periodic boundary conditions. Our framework enables the freedom to choose the flow base distributions, drastically simplifying the problem of learning crystal structures compared with diffusion models. In addition to standard benchmarks, we validate FlowMM's generated structures with quantum chemistry calculations, demonstrating that it is about 3x more efficient, in terms of integration steps, at finding stable materials compared to previous open methods.

==> docs/fbee9dc1-ac76-4c58-8f7f-d95a457e05ae <==
{"id":"r0.11545203543311422","lines":[{"blocks":[{"text":"\\diagram","type":"composite","elements":{"de38434228352009847":{"id":"de38434228352009847","lines":[{"blocks":[{"id":"n0.482039927395399","text":"Unit Cell"}],"id":"n0.7715602892551683"}],"shape":{"data":{"p":{"x":17,"y":30.525000000000006}},"anchor":"left-top"},"isTextMode":true},"de9516767649770048":{"id":"de9516767649770048","lines":[{"blocks":[{"text":"Coordinates","style":{"fontName":"ptm"},"id":"n0.692076642080917"}],"id":"n0.7549554914149974"}],"shape":{"data":{"p":{"x":9,"y":145.07635147904725}},"anchor":"left-top"},"isTextMode":true},"de557328358016191":{"id":"de557328358016191","lines":[{"blocks":[{"text":"Atom Types","style":{"fontName":"ptm"},"id":"n0.3759922322733731"}],"id":"n0.7626531649960717"}],"shape":{"data":{"p":{"x":8.5,"y":247.6250000000001}},"anchor":"left-top"},"isTextMode":true},"de6786195703949887":{"id":"de6786195703949887","lines":[{"blocks":[{"id":"n0.3811374368005922","text":"Quantize"}],"id":"n0.5255579729945805"}],"shape":{"data":{"p":{"x":550.5142857142857,"y":205.04285714285717}},"anchor":"left-top"},"isTextMode":true},"de26096050462067666":{"id":"de26096050462067666","lines":[{"blocks":[{"id":"n0.4875542827944306","text":"\\math-container","type":"composite","elements":{"mathValue":{"id":"n0.9881159137645816","lines":[{"id":"n0.7647413331490553","blocks":[{"id":"n0.5130480762618463","text":"l"},{"id":"n0.09705177973117651","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.28298269368906936","lines":[{"id":"n0.15612560108661278","blocks":[{"id":"n0.948308935458142","text":"0"}]}]}}}]}]}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"}}],"id":"n0.8437617317729482"}],"shape":{"data":{"p":{"x":89.80271175986559,"y":74.50000190734863},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true,"isInGroup":true},"de5750339631948558":{"id":"de5750339631948558","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"l","id":"n0.9295120206406631"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.08705089547957834","text":"0.5"}],"id":"n0.6129339953097606"}],"id":"n0.5387682846628419"}},"id":"n0.24284915356047465"}],"id":"n0.9179584053928864"}],"id":"n0.3049519782747554"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.6912173126434811"}],"id":"n0.4485347923793579"}],"shape":{"data":{"p":{"x":252.228982260274,"y":74},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true,"isInGroup":true},"de3663255819035478":{"id":"de3663255819035478","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"text":"l","id":"n0.010062475073193022"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.8636623268775581","text":"1"}],"id":"n0.11454956193779098"}],"id":"n0.21652082767140857"}},"id":"n0.3564192572390308"}],"id":"n0.5272304859636416"}],"id":"n0.5908699382670703"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.8824301885272958"}],"id":"n0.021363193106516354"}],"shape":{"data":{"p":{"x":425.99411302504905,"y":74},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true,"isInGroup":true},"de9194988570725868":{"id":"de9194988570725868","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"id":"n0.4092280412000038","text":"f"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"0","id":"n0.5599131410320568"}],"id":"n0.6633000117315897"}],"id":"n0.4999229132128131"}},"id":"n0.014332351837692103"}],"id":"n0.48338729117129575"}],"id":"n0.5184187873440456"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.5870054258517743"}],"id":"n0.7868418524096068"}],"shape":{"data":{"p":{"x":88.56044405873507,"y":177.00000190734863},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true,"isInGroup":true},"de6422214907510975":{"id":"de6422214907510975","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"id":"n0.2168276048405049","text":"f"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"0.5","id":"n0.8442820939407893"}],"id":"n0.8648280856032193"}],"id":"n0.5938938396556013"}},"id":"n0.5060537504549842"}],"id":"n0.5858137048252743"}],"id":"n0.22589745264712024"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.6814999591244322"}],"id":"n0.9265051458743963"}],"shape":{"data":{"p":{"x":250.9192989490785,"y":177},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true,"isInGroup":true},"de40247072652814864":{"id":"de40247072652814864","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"id":"n0.030440482069726826","text":"f"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"1","id":"n0.21111875275250847"}],"id":"n0.4515686820941256"}],"id":"n0.6971567831517298"}},"id":"n0.8735150127595435"}],"id":"n0.8308877204015594"}],"id":"n0.019813186594315635"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.8834138156388776"}],"id":"n0.15664014926903924"}],"shape":{"data":{"p":{"x":425.16123427867905,"y":176.42537747658662},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true,"isInGroup":true},"de1458711573254381":{"id":"de1458711573254381","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"id":"n0.055127974469613816","text":"a"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"0","id":"n0.8475494694020962"}],"id":"n0.26620421564821384"}],"id":"n0.20746942318518813"}},"id":"n0.10145646699371591"}],"id":"n0.845244218899275"}],"id":"n0.39269598066897804"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.7844677512565219"}],"id":"n0.5973118789195397"}],"shape":{"data":{"p":{"x":89.58783879786456,"y":273.00000190734863},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true,"isInGroup":true},"de050448089853140754":{"id":"de050448089853140754","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"id":"n0.2627000115401452","text":"a"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"0.5","id":"n0.8262128251245267"}],"id":"n0.0961057338600304"}],"id":"n0.32369430073055905"}},"id":"n0.4724106712791951"}],"id":"n0.4803429579406915"}],"id":"n0.13136638874332363"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.8258892932129631"}],"id":"n0.7742713936506675"}],"shape":{"data":{"p":{"x":252.01410929827296,"y":273},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true,"isInGroup":true},"de3393505212777461":{"id":"de3393505212777461","lines":[{"blocks":[{"text":"\\math-container","type":"composite","elements":{"mathValue":{"lines":[{"blocks":[{"id":"n0.7011795141078814","text":"a"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"1","id":"n0.711754398155553"}],"id":"n0.40458525324709993"}],"id":"n0.8360269105230291"}},"id":"n0.005604614063072777"}],"id":"n0.8064118902897581"}],"id":"n0.32702632093030903"}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"},"id":"n0.44931422860999515"}],"id":"n0.8429210146278285"}],"shape":{"data":{"p":{"x":426.1886290178085,"y":272.4253774765866},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isTextMode":true,"isInGroup":true}},"connections":[],"intersections":{"id":"di5020895009340935","items":[],"style":{}},"shapes":[{"id":"dg4159956227132138","entities":[{"id":"dp8400745450217539","type":"ellipse","data":{"p1":{"x":490.9125672317462,"y":140.19690592579332},"p2":{"x":496.1240086173087,"y":145.4083473113556}},"style":{"fillColor":[74,74,74,1],"strokeColor":"none"}},{"id":"dp21040904668675164","type":"ellipse","data":{"p1":{"x":467.4183642640474,"y":140.19690592579332},"p2":{"x":472.6298056496098,"y":145.4083473113556}},"style":{"fillColor":[74,74,74,1],"strokeColor":"none"}},{"id":"dp6358614266316633","type":"doc-pie","data":{"p1":{"x":443.92416129634864,"y":140.19690592579332},"p2":{"x":449.13560268191094,"y":145.4083473113556},"angle2":86.94999999999999,"angle1":271.06},"style":{"fillColor":[74,74,74,1],"strokeColor":"none"}},{"id":"dp7124293006400064","type":"doc-pie","data":{"p1":{"x":443.92416129634864,"y":163.69110889349216},"p2":{"x":449.13560268191094,"y":168.90255027905445},"angle2":88.18,"angle1":272.46},"style":{"fillColor":[74,74,74,1],"strokeColor":"none"}},{"id":"dp7924437366810437","type":"doc-pie","data":{"p1":{"x":443.92416129634864,"y":187.18531186119097},"p2":{"x":449.13560268191094,"y":192.3967532467533},"angle2":358.4,"angle1":267.43},"style":{"fillColor":[74,74,74,1],"strokeColor":"none"}},{"id":"dp6830436971060734","type":"doc-pie","data":{"p1":{"x":467.4183642640474,"y":187.18531186119097},"p2":{"x":472.6298056496098,"y":192.3967532467533},"angle2":358.4,"angle1":180.06},"style":{"fillColor":[74,74,74,1],"strokeColor":"none"}},{"id":"dp7884552096336777","type":"doc-pie","data":{"p1":{"x":490.9125672317462,"y":187.18531186119097},"p2":{"x":496.1240086173087,"y":192.3967532467533},"angle2":3.480000000000018,"angle1":175.79},"style":{"fillColor":[74,74,74,1],"strokeColor":"none"}},{"id":"dp7730539603602298","type":"doc-pie","data":{"p1":{"x":514.406770199445,"y":187.18531186119097},"p2":{"x":519.6182115850074,"y":192.3967532467533},"angle2":268.34,"angle1":175.51},"style":{"fillColor":[74,74,74,1],"strokeColor":"none"}},{"id":"dp49291163034215524","type":"doc-pie","data":{"p1":{"x":514.406770199445,"y":163.69110889349216},"p2":{"x":519.6182115850074,"y":168.90255027905445},"angle2":268.9,"angle1":87.99000000000001},"style":{"fillColor":[74,74,74,1],"strokeColor":"none"}},{"id":"dp8960303509007508","type":"doc-pie","data":{"p1":{"x":514.406770199445,"y":140.19690592579332},"p2":{"x":519.6182115850074,"y":145.4083473113556},"angle2":271.42,"angle1":88.84000000000003},"style":{"fillColor":[74,74,74,1],"strokeColor":"none"}},{"id":"dp3749413214120543","type":"doc-pie","data":{"p1":{"x":514.406770199445,"y":116.70270295809446},"p2":{"x":519.6182115850074,"y":121.91414434365677},"angle2":181.16,"angle1":89.26999999999998},"style":{"fillColor":[74,74,74,1],"strokeColor":"none"}},{"id":"dp2397490181000803","type":"doc-pie","data":{"p1":{"x":490.9125672317462,"y":116.70270295809446},"p2":{"x":496.1240086173087,"y":121.91414434365677},"angle2":181.16},"style":{"fillColor":[74,74,74,1],"strokeColor":"none"}},{"id":"dp9894564895969535","type":"doc-pie","data":{"p1":{"x":467.4183642640474,"y":116.70270295809446},"p2":{"x":472.6298056496098,"y":121.91414434365677},"angle2":181.16},"style":{"fillColor":[74,74,74,1],"strokeColor":"none"}},{"id":"dp39955742954806306","type":"doc-pie","data":{"p1":{"x":443.92416129634864,"y":116.70270295809446},"p2":{"x":449.13560268191094,"y":121.91414434365677},"angle2":90.95999999999998},"style":{"fillColor":[74,74,74,1],"strokeColor":"none"}},{"id":"dp9409623648512395","type":"rectangle","data":{"p1":{"x":470.0240849568287,"y":142.80262661857446},"p2":{"x":493.51828792452744,"y":166.2968295862733}}},{"id":"dp048264694838207944","type":"rectangle","data":{"p1":{"x":493.51828792452744,"y":142.80262661857446},"p2":{"x":517.0124908922262,"y":166.2968295862733}}},{"id":"dp8205962398408095","type":"rectangle","data":{"p1":{"x":493.51828792452744,"y":119.30842365087561},"p2":{"x":517.0124908922262,"y":142.80262661857446}}},{"id":"dp42220505436902367","type":"rectangle","data":{"p1":{"x":470.0240849568286,"y":119.30842365087561},"p2":{"x":493.51828792452744,"y":142.80262661857446}}},{"id":"dp9280130060308558","type":"rectangle","data":{"p1":{"x":446.5298819891299,"y":119.30842365087561},"p2":{"x":470.0240849568286,"y":142.80262661857446}}},{"id":"dp6234514853516018","type":"rectangle","data":{"p1":{"x":446.5298819891299,"y":142.80262661857446},"p2":{"x":470.0240849568286,"y":166.2968295862733}}},{"id":"dp2347261077374947","type":"rectangle","data":{"p1":{"x":493.51828792452744,"y":166.2968295862733},"p2":{"x":517.0124908922262,"y":189.79103255397214}}},{"id":"dp0706553094125868","type":"rectangle","data":{"p1":{"x":470.0240849568286,"y":166.2968295862733},"p2":{"x":493.51828792452744,"y":189.79103255397214}}},{"id":"dp8323106742812814","type":"rectangle","data":{"p1":{"x":446.5298819891299,"y":166.2968295862733},"p2":{"x":470.0240849568286,"y":189.79103255397214}}},{"id":"dp39737458654790014","type":"ellipse","data":{"p1":{"x":490.9125672317462,"y":163.69110889349216},"p2":{"x":496.1240086173087,"y":168.90255027905445}},"style":{"fillColor":[70,19,116,1],"strokeColor":"none"}},{"id":"dp79858141987566","type":"ellipse","data":{"p1":{"x":467.4183642640474,"y":163.69110889349216},"p2":{"x":472.6298056496098,"y":168.90255027905445}},"style":{"fillColor":[70,19,116,1],"strokeColor":"none"}},{"id":"dp7692516358665367","type":"ellipse","data":{"p1":{"x":480.1052338666049,"y":152.8837755283507},"p2":{"x":483.43713901475115,"y":156.21568067649704}},"style":{"fillColor":[49,239,2,1],"strokeColor":"none"}},{"id":"dp3124953841285023","type":"ellipse","data":{"p1":{"x":456.61103089890605,"y":152.8837755283507},"p2":{"x":459.94293604705234,"y":156.21568067649704}},"style":{"fillColor":[155,155,155,1],"strokeColor":"none"}},{"id":"dp24518081072608755","type":"ellipse","data":{"p1":{"x":456.61103089890605,"y":129.38957256065186},"p2":{"x":459.94293604705234,"y":132.7214777087982}},"style":{"fillColor":[155,155,155,1],"strokeColor":"none"}},{"id":"dp6512722780506042","type":"ellipse","data":{"p1":{"x":480.1052338666049,"y":129.38957256065186},"p2":{"x":483.43713901475115,"y":132.7214777087982}},"style":{"fillColor":[155,155,155,1],"strokeColor":"none"}},{"id":"dp8096272159566131","type":"ellipse","data":{"p1":{"x":503.59943683430373,"y":129.38957256065186},"p2":{"x":506.9313419824501,"y":132.7214777087982}},"style":{"fillColor":[155,155,155,1],"strokeColor":"none"}},{"id":"dp5294486202541866","type":"ellipse","data":{"p1":{"x":503.59943683430373,"y":152.8837755283507},"p2":{"x":506.9313419824501,"y":156.21568067649704}},"style":{"fillColor":[155,155,155,1],"strokeColor":"none"}},{"id":"dp18981927277776656","type":"ellipse","data":{"p1":{"x":503.59943683430373,"y":176.37797849604954},"p2":{"x":506.9313419824501,"y":179.7098836441959}},"style":{"fillColor":[155,155,155,1],"strokeColor":"none"}},{"id":"dp05878314006666474","type":"ellipse","data":{"p1":{"x":480.1052338666049,"y":176.37797849604954},"p2":{"x":483.43713901475115,"y":179.7098836441959}},"style":{"fillColor":[155,155,155,1],"strokeColor":"none"}},{"id":"dp3128735346325766","type":"ellipse","data":{"p1":{"x":456.61103089890605,"y":176.37797849604954},"p2":{"x":459.94293604705234,"y":179.7098836441959}},"style":{"fillColor":[155,155,155,1],"strokeColor":"none"}}]},{"id":"dg1518255790337808","entities":[{"id":"dp2545087392798866","type":"rectangle","data":{"p1":{"x":325.45049131435786,"y":120.0684807320167},"p2":{"x":348.9446942820567,"y":143.56268369971554}}},{"id":"dp3421102956727238","type":"ellipse","data":{"p1":{"x":318.8293977507338,"y":134.93390370066976},"p2":{"x":324.04083913629614,"y":140.14534508623206}},"style":{"fillColor":[74,74,74,1],"strokeColor":"none"}},{"id":"dp9705433765311313","type":"ellipse","data":{"p1":{"x":303.4513739900581,"y":138.52210924482745},"p2":{"x":308.66281537562037,"y":143.73355063038974}},"style":{"fillColor":[74,74,74,1],"strokeColor":"none"}},{"id":"dp41070589738478547","type":"ellipse","data":{"p1":{"x":310.3714846823621,"y":129.89332924578167},"p2":{"x":313.70338983050846,"y":133.22523439392808}},"style":{"fillColor":[155,155,155,1],"strokeColor":"none"}},{"id":"dp3825049329209165","type":"circle","data":{"p1":{"x":342.4090341837697,"y":134.9339037006697},"p2":{"x":347.620475569332,"y":140.145345086232}},"style":{"fillColor":[74,74,74,1],"strokeColor":"none"}},{"id":"dp46071117988137833","type":"ellipse","data":{"p1":{"x":327.03101042309396,"y":138.5221092448274},"p2":{"x":332.24245180865626,"y":143.73355063038974}},"style":{"fillColor":[74,74,74,1],"strokeColor":"none"}},{"id":"dp6664725237188125","type":"ellipse","data":{"p1":{"x":333.95112111539805,"y":129.89332924578167},"p2":{"x":337.2830262635444,"y":133.22523439392802}},"style":{"fillColor":[155,155,155,1],"strokeColor":"none"}},{"id":"dp9810022284768984","type":"ellipse","data":{"p1":{"x":295.420628248372,"y":135.1047706313439},"p2":{"x":300.6320696339343,"y":140.3162120169062}},"style":{"fillColor":[74,74,74,1],"strokeColor":"none"}},{"id":"dp32963180815192916","type":"circle","data":{"p1":{"x":280.0426044876963,"y":138.6929761755016},"p2":{"x":285.2540458732586,"y":143.9044175610639}},"style":{"fillColor":[74,74,74,1],"strokeColor":"none"}},{"id":"dp32489645314495896","type":"ellipse","data":{"p1":{"x":286.9627151800003,"y":130.06419617645588},"p2":{"x":290.29462032814666,"y":133.39610132460223}},"style":{"fillColor":[155,155,155,1],"strokeColor":"none"}},{"id":"dp31182578607236744","type":"ellipse","data":{"p1":{"x":294.77987725834373,"y":159.28244132173944},"p2":{"x":299.991318643906,"y":164.4938827073018}},"style":{"fillColor":[74,74,74,1],"strokeColor":"none"}},{"id":"dp2546500404406069","type":"circle","data":{"p1":{"x":279.53000369567377,"y":162.27261260853754},"p2":{"x":284.74144508123607,"y":167.48405399409984}},"style":{"fillColor":[74,74,74,1],"strokeColor":"none"}},{"id":"dp6121119942112501","type":"circle","data":{"p1":{"x":286.4501143879778,"y":153.64383260949177},"p2":{"x":289.78201953612415,"y":156.97573775763811}},"style":{"fillColor":[155,155,155,1],"strokeColor":"none"}},{"id":"dp25522263200726236","type":"ellipse","data":{"p1":{"x":295.0788943870237,"y":181.92230963606738},"p2":{"x":300.290335772586,"y":187.13375102162973}},"style":{"fillColor":[74,74,74,1],"strokeColor":"none"}},{"id":"dp10471341347701069","type":"circle","data":{"p1":{"x":279.700870626348,"y":185.51051518022513},"p2":{"x":284.9123120119103,"y":190.72195656578742}},"style":{"fillColor":[74,74,74,1],"strokeColor":"none"}},{"id":"dp17794078126747737","type":"ellipse","data":{"p1":{"x":286.620981318652,"y":176.88173518117935},"p2":{"x":289.95288646679836,"y":180.21364032932576}},"style":{"fillColor":[155,155,155,1],"strokeColor":"none"}},{"id":"dp31443374196049945","type":"ellipse","data":{"p1":{"x":318.65853082005964,"y":182.0931765667416},"p2":{"x":323.86997220562193,"y":187.3046179523039}},"style":{"fillColor":[74,74,74,1],"strokeColor":"none"}},{"id":"dp5191335645921329","type":"ellipse","data":{"p1":{"x":303.28050705938386,"y":185.68138211089928},"p2":{"x":308.4919484449462,"y":190.89282349646157}},"style":{"fillColor":[74,74,74,1],"strokeColor":"none"}},{"id":"dp001184681820838085","type":"circle","data":{"p1":{"x":310.20061775168796,"y":177.05260211185356},"p2":{"x":313.5325228998343,"y":180.3845072599999}},"style":{"fillColor":[155,155,155,1],"strokeColor":"none"}},{"id":"dp6609807226887363","type":"circle","data":{"p1":{"x":342.23816725309547,"y":181.92230963606738},"p2":{"x":347.4496086386578,"y":187.13375102162973}},"style":{"fillColor":[74,74,74,1],"strokeColor":"none"}},{"id":"dp42485413221722657","type":"circle","data":{"p1":{"x":326.8601434924198,"y":185.51051518022513},"p2":{"x":332.0715848779821,"y":190.72195656578742}},"style":{"fillColor":[74,74,74,1],"strokeColor":"none"}},{"id":"dp8830561824046261","type":"ellipse","data":{"p1":{"x":333.78025418472384,"y":176.88173518117935},"p2":{"x":337.11215933287025,"y":180.21364032932576}},"style":{"fillColor":[155,155,155,1],"strokeColor":"none"}},{"id":"dp7808450801129825","type":"ellipse","data":{"p1":{"x":342.23816725309547,"y":158.51354013370565},"p2":{"x":347.4496086386578,"y":163.72498151926794}},"style":{"fillColor":[74,74,74,1],"strokeColor":"none"}},{"id":"dp8491315825562245","type":"ellipse","data":{"p1":{"x":326.8601434924198,"y":162.10174567786333},"p2":{"x":332.0715848779821,"y":167.3131870634257}},"style":{"fillColor":[74,74,74,1],"strokeColor":"none"}},{"id":"dp8923876262094119","type":"ellipse","data":{"p1":{"x":333.78025418472384,"y":153.47296567881762},"p2":{"x":337.11215933287025,"y":156.80487082696396}},"style":{"fillColor":[155,155,155,1],"strokeColor":"none"}},{"id":"dp8391692544118527","type":"rectangle","data":{"p1":{"x":301.956288346659,"y":143.56268369971554},"p2":{"x":325.45049131435786,"y":167.0568866674144}}},{"id":"dp574029281887789","type":"circle","data":{"p1":{"x":318.145930028037,"y":158.5135401337057},"p2":{"x":323.3573714135993,"y":163.724981519268}},"style":{"fillColor":[70,19,116,1],"strokeColor":"none"}},{"id":"dp5125214788511638","type":"ellipse","data":{"p1":{"x":303.451373990058,"y":162.27261260853754},"p2":{"x":308.66281537562037,"y":167.48405399409984}},"style":{"fillColor":[80,227,194,1],"strokeColor":"none"}},{"id":"dp5103257388758717","type":"circle","data":{"p1":{"x":310.3714846823621,"y":153.64383260949177},"p2":{"x":313.70338983050846,"y":156.97573775763811}},"style":{"fillColor":[49,239,2,1],"strokeColor":"none"}},{"id":"dp47860318193410967","type":"rectangle","data":{"p1":{"x":325.45049131435786,"y":143.56268369971554},"p2":{"x":348.9446942820567,"y":167.0568866674144}}},{"id":"dp7831738220400106","type":"rectangle","data":{"p1":{"x":325.45049131435786,"y":167.0568866674144},"p2":{"x":348.9446942820567,"y":190.55108963511321}}},{"id":"dp6953424219864803","type":"rectangle","data":{"p1":{"x":301.956288346659,"y":167.0568866674144},"p2":{"x":325.45049131435786,"y":190.55108963511321}}},{"id":"dp8308846572381594","type":"rectangle","data":{"p1":{"x":278.46208537896024,"y":120.0684807320167},"p2":{"x":301.956288346659,"y":143.56268369971554}}},{"id":"dp28545441462225374","type":"rectangle","data":{"p1":{"x":278.46208537896024,"y":143.56268369971554},"p2":{"x":301.956288346659,"y":167.0568866674144}}},{"id":"dp6025475300404095","type":"rectangle","data":{"p1":{"x":278.46208537896024,"y":167.0568866674144},"p2":{"x":301.956288346659,"y":190.55108963511321}}},{"id":"dp9718636477471387","type":"rectangle","data":{"p1":{"x":301.956288346659,"y":120.0684807320167},"p2":{"x":325.45049131435786,"y":143.56268369971554}}}]},{"id":"dg2798664159210582","entities":[{"id":"dp22398449325484315","type":"rectangle","data":{"p1":{"x":134.09188156699798,"y":142.99181676904135},"p2":{"x":157.58608453469682,"y":166.48601973674022}}},{"id":"dp8825507124617908","type":"circle","data":{"p1":{"x":148.6155706743027,"y":144.4441856797718},"p2":{"x":153.827012059865,"y":149.65562706533413}},"style":{"fillColor":[245,166,35,1],"strokeColor":"none"}},{"id":"dp22890518704696516","type":"ellipse","data":{"p1":{"x":134.56176562635196,"y":159.3096086484249},"p2":{"x":139.77320701191425,"y":164.52105003398722}},"style":{"fillColor":[80,227,194,1],"strokeColor":"none"}},{"id":"dp25009198274570577","type":"circle","data":{"p1":{"x":148.23112008028585,"y":158.45527399505409},"p2":{"x":151.5630252284322,"y":161.78717914320043}},"style":{"fillColor":[49,239,2,1],"strokeColor":"none"}},{"id":"dp12478046372076346","type":"rectangle","data":{"p1":{"x":157.58608453469682,"y":142.99181676904135},"p2":{"x":181.08028750239566,"y":166.48601973674022}}},{"id":"dp46794678654424837","type":"rectangle","data":{"p1":{"x":157.58608453469682,"y":119.49761380134252},"p2":{"x":181.08028750239566,"y":142.99181676904135}}},{"id":"dp24381546225097983","type":"rectangle","data":{"p1":{"x":134.09188156699798,"y":119.49761380134252},"p2":{"x":157.58608453469682,"y":142.99181676904135}}},{"id":"dp08280531902609733","type":"rectangle","data":{"p1":{"x":110.59767859929914,"y":119.49761380134252},"p2":{"x":134.09188156699798,"y":142.99181676904135}}},{"id":"dp5626994051655088","type":"rectangle","data":{"p1":{"x":110.59767859929914,"y":142.99181676904135},"p2":{"x":134.09188156699798,"y":166.48601973674022}}},{"id":"dp5605341243804345","type":"ellipse","data":{"p1":{"x":172.02434017666442,"y":121.03541617741007},"p2":{"x":177.23578156222675,"y":126.24685756297237}},"style":{"fillColor":[74,74,74,1],"strokeColor":"none"}},{"id":"dp042028556432959","type":"circle","data":{"p1":{"x":157.9705351287137,"y":135.90083914606316},"p2":{"x":163.181976514276,"y":141.11228053162546}},"style":{"fillColor":[74,74,74,1],"strokeColor":"none"}},{"id":"dp46000932925040416","type":"circle","data":{"p1":{"x":171.6398895826476,"y":135.04650449269232},"p2":{"x":174.97179473079396,"y":138.37840964083867}},"style":{"fillColor":[155,155,155,1],"strokeColor":"none"}},{"id":"dp7835684677530084","type":"rectangle","data":{"p1":{"x":157.58608453469682,"y":166.48601973674022},"p2":{"x":181.08028750239566,"y":189.98022270443903}}},{"id":"dp29496919682354394","type":"rectangle","data":{"p1":{"x":134.09188156699798,"y":166.48601973674022},"p2":{"x":157.58608453469682,"y":189.98022270443903}}},{"id":"dp7174581534927671","type":"rectangle","data":{"p1":{"x":110.59767859929914,"y":166.48601973674022},"p2":{"x":134.09188156699798,"y":189.98022270443903}}},{"id":"dp43683740412206173","type":"ellipse","data":{"p1":{"x":172.02434017666448,"y":144.78591954112017},"p2":{"x":177.23578156222678,"y":149.9973609266825}},"style":{"fillColor":[74,74,74,1],"strokeColor":"none"}},{"id":"dp3044796814572339","type":"circle","data":{"p1":{"x":157.97053512871375,"y":159.65134250977326},"p2":{"x":163.18197651427604,"y":164.86278389533555}},"style":{"fillColor":[74,74,74,1],"strokeColor":"none"}},{"id":"dp9916659444483189","type":"ellipse","data":{"p1":{"x":171.63988958264764,"y":158.79700785640242},"p2":{"x":174.971794730794,"y":162.1289130045488}},"style":{"fillColor":[155,155,155,1],"strokeColor":"none"}},{"id":"dp5636403711493236","type":"ellipse","data":{"p1":{"x":148.4524704222956,"y":121.00434946274206},"p2":{"x":153.66391180785786,"y":126.21579084830437}},"style":{"fillColor":[74,74,74,1],"strokeColor":"none"}},{"id":"dp2330769702052018","type":"ellipse","data":{"p1":{"x":134.39866537434483,"y":135.86977243139515},"p2":{"x":139.61010675990715,"y":141.08121381695744}},"style":{"fillColor":[74,74,74,1],"strokeColor":"none"}},{"id":"dp029872855298380907","type":"circle","data":{"p1":{"x":148.06801982827875,"y":135.0154377780243},"p2":{"x":151.3999249764251,"y":138.34734292617065}},"style":{"fillColor":[155,155,155,1],"strokeColor":"none"}},{"id":"dp609810426867218","type":"ellipse","data":{"p1":{"x":124.95826745459672,"y":121.00434946274206},"p2":{"x":130.169708840159,"y":126.21579084830437}},"style":{"fillColor":[74,74,74,1],"strokeColor":"none"}},{"id":"dp8781841375927617","type":"ellipse","data":{"p1":{"x":110.90446240664596,"y":135.86977243139515},"p2":{"x":116.11590379220827,"y":141.08121381695744}},"style":{"fillColor":[74,74,74,1],"strokeColor":"none"}},{"id":"dp5540488888986916","type":"circle","data":{"p1":{"x":124.57381686057988,"y":135.0154377780243},"p2":{"x":127.90572200872623,"y":138.34734292617065}},"style":{"fillColor":[155,155,155,1],"strokeColor":"none"}},{"id":"dp9977607216778819","type":"ellipse","data":{"p1":{"x":124.95826745459672,"y":144.615052610446},"p2":{"x":130.169708840159,"y":149.8264939960083}},"style":{"fillColor":[74,74,74,1],"strokeColor":"none"}},{"id":"dp5427105391066811","type":"ellipse","data":{"p1":{"x":110.90446240664596,"y":159.4804755790991},"p2":{"x":116.11590379220827,"y":164.6919169646614}},"style":{"fillColor":[74,74,74,1],"strokeColor":"none"}},{"id":"dp7913366253908356","type":"circle","data":{"p1":{"x":124.57381686057988,"y":158.62614092572827},"p2":{"x":127.90572200872623,"y":161.9580460738746}},"style":{"fillColor":[155,155,155,1],"strokeColor":"none"}},{"id":"dp24310809293534752","type":"ellipse","data":{"p1":{"x":124.95826745459672,"y":168.69175647817045},"p2":{"x":130.16970884015902,"y":173.90319786373277}},"style":{"fillColor":[74,74,74,1],"strokeColor":"none"}},{"id":"dp9778467486558906","type":"ellipse","data":{"p1":{"x":110.90446240664596,"y":183.55717944682354},"p2":{"x":116.11590379220827,"y":188.76862083238584}},"style":{"fillColor":[74,74,74,1],"strokeColor":"none"}},{"id":"dp6916046689241","type":"ellipse","data":{"p1":{"x":124.57381686057988,"y":182.7028447934527},"p2":{"x":127.90572200872626,"y":186.03474994159905}},"style":{"fillColor":[155,155,155,1],"strokeColor":"none"}},{"id":"dp8833791806758606","type":"ellipse","data":{"p1":{"x":148.56897060230068,"y":168.8470900515106},"p2":{"x":153.78041198786298,"y":174.05853143707293}},"style":{"fillColor":[74,74,74,1],"strokeColor":"none"}},{"id":"dp9122521554260272","type":"ellipse","data":{"p1":{"x":134.51516555434995,"y":183.7125130201637},"p2":{"x":139.72660693991224,"y":188.92395440572602}},"style":{"fillColor":[74,74,74,1],"strokeColor":"none"}},{"id":"dp5301871952072248","type":"ellipse","data":{"p1":{"x":148.18452000828387,"y":182.85817836679286},"p2":{"x":151.5164251564302,"y":186.1900835149392}},"style":{"fillColor":[155,155,155,1],"strokeColor":"none"}},{"id":"dp18550291718233192","type":"ellipse","data":{"p1":{"x":172.02434017666448,"y":168.69175647817045},"p2":{"x":177.23578156222678,"y":173.90319786373277}},"style":{"fillColor":[74,74,74,1],"strokeColor":"none"}},{"id":"dp40404913558598143","type":"circle","data":{"p1":{"x":157.97053512871375,"y":183.55717944682354},"p2":{"x":163.18197651427604,"y":188.76862083238584}},"style":{"fillColor":[74,74,74,1],"strokeColor":"none"}},{"id":"dp5277477274803499","type":"circle","data":{"p1":{"x":171.63988958264764,"y":182.7028447934527},"p2":{"x":174.971794730794,"y":186.03474994159905}},"style":{"fillColor":[155,155,155,1],"strokeColor":"none"}}]},{"id":"dg9444558059099066","entities":[{"id":"da011198597682665623","data":[{"x":104.98586323254692,"y":196},{"x":441.80536253410315,"y":195.5}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"dp20379207278438694","type":"ellipse","data":{"p1":{"x":102.59122576665008,"y":192.95},"p2":{"x":107.38050069844378,"y":199.05}},"style":{"fillColor":[0,0,0,1],"strokeColor":"none"}},{"id":"dp5245921242711713","type":"ellipse","data":{"p1":{"x":271.0009754174282,"y":192.7},"p2":{"x":275.7902503492219,"y":198.8}},"style":{"fillColor":[0,0,0,1],"strokeColor":"none"}},{"id":"dp10456307634900042","type":"ellipse","data":{"p1":{"x":439.4107250682064,"y":192.45},"p2":{"x":444.2,"y":198.55}},"style":{"fillColor":[0,0,0,1],"strokeColor":"none"}},{"id":"dl1851142551808389","linkedId":"de9194988570725868"},{"id":"dl569018346142883","linkedId":"de6422214907510975"},{"id":"dl902831119410888","linkedId":"de40247072652814864"}],"data":{"rotation":0}},{"id":"dg8001690982993437","entities":[{"id":"dp07879390665166475","type":"square","data":{"p1":{"x":553.6142857142859,"y":257.2},"p2":{"x":583.8142857142857,"y":287.40000000000003}},"style":{"fillColor":[49,239,2,0.34]}},{"id":"dp3397788450897188","type":"square","data":{"p1":{"x":583.8142857142857,"y":226.80000000000024},"p2":{"x":614.0142857142857,"y":257.00000000000017}},"style":{"fillColor":[70,19,116,0.27]}},{"id":"dp7644914991214977","type":"square","data":{"p1":{"x":553.8142857142858,"y":227.00000000000009},"p2":{"x":614.0142857142857,"y":287.2000000000001}}},{"id":"dp4877788916079546","type":"circle","data":{"p1":{"x":590.6642857142858,"y":236.75000000000009},"p2":{"x":598.8642857142859,"y":244.95000000000013}},"style":{"fillColor":[70,19,116,1],"strokeColor":"none"}},{"id":"dp3957429948015003","type":"circle","data":{"p1":{"x":560.2714285714286,"y":279.0142857142858},"p2":{"x":565.5142857142857,"y":284.2571428571429}},"style":{"fillColor":[49,239,2,1],"strokeColor":"none"}},{"id":"dp8313935758892737","type":"circle","data":{"p1":{"x":603.4142857142858,"y":228.10000000000016},"p2":{"x":611.6142857142859,"y":236.3000000000002}},"style":{"fillColor":[70,19,116,1],"strokeColor":"none"}},{"id":"dp6101631138783612","type":"square","data":{"p1":{"x":553.6142857142859,"y":227.00000000000009},"p2":{"x":583.8142857142857,"y":257.2}},"style":{"fillColor":[80,227,194,0.25]}},{"id":"dp7143521300648701","type":"square","data":{"p1":{"x":583.8142857142857,"y":257.00000000000017},"p2":{"x":614.0142857142857,"y":287.2000000000001}},"style":{"fillColor":[245,166,35,0.34]}}]},{"id":"dg8717119997142555","entities":[{"id":"dp1299189188692209","type":"square","data":{"p1":{"x":451.5711864406781,"y":226.20000000000007},"p2":{"x":481.7711864406779,"y":256.4}},"style":{"fillColor":[80,227,194,0.25],"strokeColor":"none"}},{"id":"dp7663804801223044","type":"square","data":{"p1":{"x":451.5711864406781,"y":256.4},"p2":{"x":481.7711864406779,"y":286.6}},"style":{"fillColor":[49,239,2,0.34],"strokeColor":"none"}},{"id":"dp02680777184913774","type":"square","data":{"p1":{"x":481.7711864406779,"y":226.00000000000023},"p2":{"x":511.97118644067797,"y":256.20000000000016}},"style":{"fillColor":[70,19,116,0.27],"strokeColor":"none"}},{"id":"dp6272819500749212","type":"square","data":{"p1":{"x":481.7711864406779,"y":256.20000000000016},"p2":{"x":511.97118644067797,"y":286.4000000000001}},"style":{"fillColor":[245,166,35,0.34],"strokeColor":"none"}},{"id":"dp9395819114314508","type":"square","data":{"p1":{"x":451.67118796655694,"y":226.20000000000007},"p2":{"x":511.8711879665569,"y":286.4000000000001}}},{"id":"dp02485350810656639","type":"circle","data":{"p1":{"x":488.52118796655697,"y":235.95000000000007},"p2":{"x":496.721187966557,"y":244.15000000000012}},"style":{"fillColor":"none","strokeColor":[0,0,0,1],"thickness":1}},{"id":"dp9890887792574536","type":"circle","data":{"p1":{"x":501.27118796655697,"y":227.30000000000015},"p2":{"x":509.471187966557,"y":235.5000000000002}},"style":{"fillColor":"none","strokeColor":[0,0,0,1],"thickness":1}},{"id":"dp38761897027622183","type":"circle","data":{"p1":{"x":458.70690143483614,"y":277.93571346827923},"p2":{"x":464.0354744982779,"y":283.26428653172104}},"style":{"fillColor":"none","strokeColor":[0,0,0,1],"thickness":1}}]},{"id":"dg09808406573791029","entities":[{"id":"dp7487119211742306","type":"square","data":{"p1":{"x":283.5676747818548,"y":225.20000000000005},"p2":{"x":313.7676747818546,"y":255.40000000000003}},"style":{"fillColor":[80,227,194,0.25],"strokeColor":"none"}},{"id":"dp9953592053833704","type":"square","data":{"p1":{"x":283.5676747818548,"y":255.40000000000003},"p2":{"x":313.7676747818546,"y":285.59999999999997}},"style":{"fillColor":[49,239,2,0.34],"strokeColor":"none"}},{"id":"dp26871264416914076","type":"square","data":{"p1":{"x":313.7676747818546,"y":225.00000000000023},"p2":{"x":343.96767478185467,"y":255.2000000000001}},"style":{"fillColor":[70,19,116,0.27],"strokeColor":"none"}},{"id":"dp3947301949534878","type":"square","data":{"p1":{"x":313.7676747818546,"y":255.2000000000001},"p2":{"x":343.96767478185467,"y":285.40000000000003}},"style":{"fillColor":[245,166,35,0.34],"strokeColor":"none"}},{"id":"dp3447737067551033","type":"square","data":{"p1":{"x":283.43910487916224,"y":225.39999999999992},"p2":{"x":343.63910487916223,"y":285.59999999999997}}},{"id":"dp5672051517655818","type":"circle","data":{"p1":{"x":305.8391048791622,"y":244.4999999999999},"p2":{"x":314.03910487916227,"y":252.69999999999993}},"style":{"fillColor":"none","strokeColor":[0,0,0,1],"thickness":1}},{"id":"dp8848705496380473","type":"circle","data":{"p1":{"x":327.8391048791623,"y":242.49999999999994},"p2":{"x":336.0391048791623,"y":250.7}},"style":{"fillColor":"none","strokeColor":[0,0,0,1],"thickness":1}},{"id":"dp23766652466511884","type":"circle","data":{"p1":{"x":300.07481834744135,"y":262.7357134682791},"p2":{"x":305.4033914108831,"y":268.0642865317208}},"style":{"fillColor":"none","strokeColor":[0,0,0,1],"thickness":1}}]},{"id":"dg08804163452177893","entities":[{"id":"dp5217378177509335","type":"square","data":{"p1":{"x":115.66755366198387,"y":224.95714285714297},"p2":{"x":145.8675536619837,"y":255.1571428571429}},"style":{"fillColor":[80,227,194,0.25],"strokeColor":"none"}},{"id":"dp5912272333140949","type":"square","data":{"p1":{"x":115.66755366198387,"y":255.1571428571429},"p2":{"x":145.8675536619837,"y":285.3571428571429}},"style":{"fillColor":[49,239,2,0.34],"strokeColor":"none"}},{"id":"dp21151007941757793","type":"square","data":{"p1":{"x":145.8675536619837,"y":224.75714285714312},"p2":{"x":176.06755366198374,"y":254.95714285714303}},"style":{"fillColor":[70,19,116,0.27],"strokeColor":"none"}},{"id":"dp14573115305733375","type":"square","data":{"p1":{"x":145.8675536619837,"y":254.95714285714303},"p2":{"x":176.06755366198374,"y":285.15714285714296}},"style":{"fillColor":[245,166,35,0.34],"strokeColor":"none"}},{"id":"dp5276776051592678","type":"square","data":{"p1":{"x":115.6104124397111,"y":224.70000000000005},"p2":{"x":175.81041243971111,"y":284.9000000000001}}},{"id":"dp8131136235081569","type":"circle","data":{"p1":{"x":145.83898386828255,"y":256.3142857142858},"p2":{"x":154.03898386828257,"y":264.51428571428585}},"style":{"fillColor":"none","strokeColor":[0,0,0,1],"thickness":1}},{"id":"dp8481680816557249","type":"circle","data":{"p1":{"x":137.95326794769795,"y":254.77142857142854},"p2":{"x":143.2818410111397,"y":260.1000016348703}},"style":{"fillColor":"none","strokeColor":[0,0,0,1],"thickness":1}},{"id":"dp053993704196168224","type":"circle","data":{"p1":{"x":140.75326958256827,"y":245.28571428571433},"p2":{"x":148.95326958256828,"y":253.48571428571438}},"style":{"fillColor":"none","strokeColor":[0,0,0,1],"thickness":1}}]},{"id":"dg729599428874798","entities":[{"id":"da033022011551236075","data":[{"x":104.98586323254692,"y":291},{"x":441.80536253410315,"y":290.5}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"dp1395760025012731","type":"ellipse","data":{"p1":{"x":102.59122576665008,"y":287.95},"p2":{"x":107.38050069844378,"y":294.05}},"style":{"fillColor":[0,0,0,1],"strokeColor":"none"}},{"id":"dp726319381151179","type":"ellipse","data":{"p1":{"x":271.0009754174282,"y":287.7},"p2":{"x":275.7902503492219,"y":293.8}},"style":{"fillColor":[0,0,0,1],"strokeColor":"none"}},{"id":"dp4129265490893306","type":"ellipse","data":{"p1":{"x":439.4107250682064,"y":287.45},"p2":{"x":444.2,"y":293.55}},"style":{"fillColor":[0,0,0,1],"strokeColor":"none"}},{"id":"dl7715197353245051","linkedId":"de1458711573254381"},{"id":"dl9312867509242624","linkedId":"de050448089853140754"},{"id":"dl8113795390165404","linkedId":"de3393505212777461"}],"data":{"rotation":0}},{"id":"dp7824533252520731","type":"image","data":{"p1":{"x":441.4322033898306,"y":7.976271186440684},"p2":{"x":522.1101694915255,"y":88.65423728813559},"url":"data-resources/a0271b71-eda9-4c8f-be71-80dc145e845c"}},{"id":"dg2742797706677358","entities":[{"id":"da08227268875179816","data":[{"x":103.0230456375495,"y":94},{"x":439.8425449391057,"y":93.5}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"dp3284436771279575","type":"ellipse","data":{"p1":{"x":100.62840817165267,"y":90.94999999999999},"p2":{"x":105.41768310344636,"y":97.05000000000001}},"style":{"fillColor":[0,0,0,1],"strokeColor":"none"}},{"id":"dp4463848114780178","type":"ellipse","data":{"p1":{"x":269.0381578224308,"y":90.69999999999999},"p2":{"x":273.8274327542245,"y":96.80000000000001}},"style":{"fillColor":[0,0,0,1],"strokeColor":"none"}},{"id":"dp31631880563682","type":"ellipse","data":{"p1":{"x":437.447907473209,"y":90.44999999999999},"p2":{"x":442.23718240500256,"y":96.55000000000001}},"style":{"fillColor":[0,0,0,1],"strokeColor":"none"}},{"id":"dl049017620482346036","linkedId":"de26096050462067666"},{"id":"dl2717162467396492","linkedId":"de5750339631948558"},{"id":"dl47565331346248674","linkedId":"de3663255819035478"}],"data":{"rotation":0}},{"id":"dp08285480526873878","type":"image","data":{"p1":{"x":273.36440677966095,"y":8.599999999999994},"p2":{"x":354.04237288135596,"y":89.2779661016949},"url":"data-resources/1681e6ef-1c47-4cd2-a255-f3e7b6ff098c"}},{"id":"dp6911709326216948","type":"image","data":{"p1":{"x":105.49999999999997,"y":7.922033898305083},"p2":{"x":186.1779661016949,"y":88.6},"url":"data-resources/2eb977fe-3b3b-4ced-b199-8b28780ac584"}}],"settings":{"grid":true,"gridBold":false,"diagramHeight":300},"id":"n0.18127256291539418"}],"id":"n0.859314095195588"}],"pageSettings":{"pageSize":{"width":675},"printedPageSize":{"presetSize":"letter","width":8.27,"height":11.69,"sizeUnit":"inch","orientation":"portrait","margin":{"left":1,"top":1,"right":1,"bottom":1,"unit":"inch"},"headerFooterModel":{"header":[{"id":"n0.42594601164397483","blocks":[]}],"footer":[{"id":"n0.9098120372096061","blocks":[]}]}}},"___version":2,"version":2,"av":206,"delayRenderCache":{"av":206,"map":{}}}
